Invert and Defend: Model-based Approximate Inversion of Generative Adversarial Networks for Secure Inference

Inferring the latent variable generating a given test sample is a challenging problem in Generative Adversarial Networks (GANs). In this paper, we propose InvGAN - a novel framework for solving the inference problem in GANs, which involves training an encoder network capable of inverting a pre-trained generator network without access to any training data. Under mild assumptions, we theoretically show that using InvGAN, we can approximately invert the generations of any latent code of a trained GAN model. Furthermore, we empirically demonstrate the superiority of our inference scheme by quantitative and qualitative comparisons with other methods that perform a similar task. We also show the effectiveness of our framework in the problem of adversarial defenses where InvGAN can successfully be used as a projection-based defense mechanism. Additionally, we show how InvGAN can be used to implement reparameterization white-box attacks on projection-based defense mechanisms. Experimental validation on several benchmark datasets demonstrate the efficacy of our method in achieving improved performance on several white-box and black-box attacks. Our code is available at https://github.com/yogeshbalaji/InvGAN.

==> figures/inversion_qualitative.tex <==
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/png/inversion_qualitative.pdf}
    \caption{Inversion visualization on CIFAR-10}
    \label{fig:inversion_vis}
\end{figure}

==> figures/roc_plot.tex <==
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.6\textwidth]{figures/png/ROC_curve.png}
    \caption{ROC plot of attack detection on CIFAR-10 under BPDA attack}
    \label{fig:roc_curve}
\end{figure}

==> tables/ablation_detection.tex <==
% \begin{table}[h!]
%     \centering
%     \caption{Performance comparison between image-level and semantic-level attack detection.} \label{table:ablation_detection}
%     \begin{tabular}{@{}lcccc@{}}
%     \toprule
%       & FGSM & CW & RP & BPDA \\
%     \midrule
%     Image-level & 0.6117 & 0.6596 & \textbf{0.6107} & \textbf{0.8156} \\
%     Semantic-level (Ours) & \textbf{0.8132} & \textbf{0.8370} & 0.5469 & 0.7807 \\
%     \bottomrule
%     \end{tabular}
% \end{table}

==> tables/blackbox.tex <==
\begin{table}[h!]
    \centering
    \caption{Black-box attack performance comparison on MNIST and Fasion-MNIST.}
    \label{table:blackbox}
    %\begin{tabular}{@{}cccccc@{}}
    \begin{tabular}{c|ccc}
    \toprule
    %\multicolumn{3}{c}{MNIST} & \multicolumn{3}{c}{Fashion-MNIST} \\
    \cmidrule(r){1-3} \cmidrule(l){4-6}
    Dataset & No Defense & DefenseGAN & InvGAN \\   
    \midrule
    MNIST & 0.6631 & 0.9398 & 0.9449 \\
    Fashion-MNIST & 0.4988 & 0.6320 & 0.6596 \\
    \bottomrule
    \end{tabular}
\end{table}
